Block Basis Factorization for Scalable Kernel Matrix Evaluation

Kernel methods are widespread in machine learning; however, they are limited by the quadratic complexity of the construction, application, and storage of kernel matrices. Low-rank matrix approximation algorithms are widely used to address this problem and reduce the arithmetic and storage cost. However, we observed that for some datasets with wide intra-class variability, the optimal kernel parameter for smaller classes yields a matrix that is less well approximated by low-rank methods. In this paper, we propose an efficient structured low-rank approximation method -- the Block Basis Factorization (BBF) -- and its fast construction algorithm to approximate radial basis function (RBF) kernel matrices. Our approach has linear memory cost and floating-point operations for many machine learning kernels. BBF works for a wide range of kernel bandwidth parameters and extends the domain of applicability of low-rank approximation methods significantly. Our empirical results demonstrate the stability and superiority over the state-of-art kernel approximation algorithms.

==> Makefile <==
name=bbf

all: $(name).pdf

$(name).pdf: $(name).tex
	pdflatex $(name)
	bibtex   $(name).aux
	pdflatex $(name)
	pdflatex $(name)

reply:
	pdflatex ReplyLetter
	pdflatex ReplyLetter

clean:
	rm -f $~ *.aux *.idx *.log *.blg *.bbl *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls *.thm
cleanless:
	rm -f $~ *.aux *.idx *.log *.blg *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls *.thm
cleanall:
	rm -f $~ *.aux *.idx *.log *.blg *.bbl *.toc *.dvi *.ps *.out *.gz \
			 *.fdb_latexmk *.fls *.thm \
	         figure/*-eps-converted-to.pdf $(name).pdf \
			 ReplyLetter.pdf
zip:
	tar cvzf $(name).tar.gz *.bib *.bbl *.tex *.pdf figure/*.eps \
		replyletterR1/* replyletterR2/*

